BoolNet: Minimizing The Energy Consumption of Binary Neural Networks

Recent works on Binary Neural Networks (BNNs) have made promising progress in narrowing the accuracy gap of BNNs to their 32-bit counterparts. However, the accuracy gains are often based on specialized model designs using additional 32-bit components. Furthermore, almost all previous BNNs use 32-bit for feature maps and the shortcuts enclosing the corresponding binary convolution blocks, which helps to effectively maintain the accuracy, but is not friendly to hardware accelerators with limited memory, energy, and computing resources. Thus, we raise the following question: How can accuracy and energy consumption be balanced in a BNN network design? We extensively study this fundamental problem in this work and propose a novel BNN architecture without most commonly used 32-bit components: \textit{BoolNet}. Experimental results on ImageNet demonstrate that BoolNet can achieve 4.6x energy reduction coupled with 1.2\% higher accuracy than the commonly used BNN architecture Bi-RealNet. Code and trained models are available at: https://github.com/hpi-xnor/BoolNet.

==> ablation_networks.tex <==
\setlength\tabcolsep{2pt}
\begin{table}[]
\caption{Our ablation study on ImageNet \cite{deng2009imagenet}.}
\begin{center}
\scriptsize
\begin{tabular}{l|cccccc|cccccc}
                          & \multicolumn{6}{c|}{ResNet} & \multicolumn{6}{c}{BoolNet} \\
 \multicolumn{1}{c|}{k=1} &
  \makecell{Top 1\\ Acc.}        & \makecell{Top 5\\ Acc.}       & \makecell{FLOPs\\($\cdot10^8$)} &
  \makecell{BOPs\\($\cdot10^9$)} & \makecell{OPs\\($\cdot10^8$)} & \makecell{Model\\ Size} &
  \makecell{Top 1\\ Acc.}        & \makecell{Top 5\\ Acc.}       & \makecell{FLOPs\\($\cdot10^8$)} &
  \makecell{BOPs\\($\cdot10^9$)} & \makecell{OPs\\($\cdot10^8$)} & \makecell{Model\\ Size} \\ \hline
Baseline (no shortcuts)       & 46.26\% & 70.84\% & 1.23 & 1.76 & 1.51 & 3.49 MB & -       & -       & -        & -        & -        & -       \\
+ Logic Shortcuts (XNOR/OR)   & 48.60\% & 72.79\% & 1.23 & 1.76 & 1.51 & 3.49 MB & 49.92\% & 74.17\% & 1.23 & 2.01 & 1.55 & 3.71 MB \\
+ Local Adaptive Binarization & 48.83\% & 73.19\% & 1.26 & 1.76 & 1.53 & 3.49 MB & 51.51\% & 75.41\% & 1.26 & 2.01 & 1.57 & 3.71 MB
\end{tabular}
\label{tab:ablation-network}
\end{center}
\end{table}


==> ablation_slices.tex <==
\setlength\tabcolsep{3pt}
\begin{table}[]
\caption{Our ablation study on ImageNet \cite{deng2009imagenet}.}
\begin{center}
\scriptsize
\begin{tabular}{c|cccccc|cccccc}
\multicolumn{1}{l|}{} & \multicolumn{6}{c|}{ResNet (with Logic Shortcuts)}           & \multicolumn{6}{c}{\scriptsize BoolNet (with Logic Shortcut and Local Adaptive Binarization)}                                  \\
k &
  \makecell{Top 1\\ Acc.}        & \makecell{Top 5\\ Acc.}       & \makecell{FLOPs\\($\cdot10^8$)} &
  \makecell{BOPs\\($\cdot10^9$)} & \makecell{OPs\\($\cdot10^8$)} & \makecell{Model\\ Size} &
  \makecell{Top 1\\ Acc.}        & \makecell{Top 5\\ Acc.}       & \makecell{FLOPs\\($\cdot10^8$)} &
  \makecell{BOPs\\($\cdot10^9$)} & \makecell{OPs\\($\cdot10^8$)} & \makecell{Model\\ Size} \\ \hline
1                     & 48.60\% & 72.79\% & 1.23 & 1.76 & 1.51 & 3.49 MB & 51.51\% & 75.41\% & 1.26 & 2.01 & 1.57 & 3.71 MB \\
4                     & 52.15\% & 75.89\% & 1.23 & 2.01 & 1.55 & 3.56 MB & xx.xx\% & xx.xx\% & 1.26 & 2.50 & 1.65 & 3.84 MB \\
8                     & 52.51\% & 76.34\% & 1.23 & 2.35 & 1.60 & 3.65 MB & -       & -       & -        & -        & -        & -      
\end{tabular}
\label{tab:ablation-slices}
\end{center}
\end{table}


==> check_list.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    %\answerTODO{}
    \answerYes{}
  \item Did you describe the limitations of your work?
    %\answerTODO{}
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    %\answerTODO{}
    \answerNA{We think there are no negative societal impacts of our work, that need considering.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    %\answerTODO{}
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    %\answerTODO{}
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    %\answerTODO{}
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    %\answerTODO{}
    \answerYes{See the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    %\answerTODO{}
    \answerYes{See the supplementary material.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    %\answerTODO{}
    \answerNo{Regarding our limited computing resources, it is too time-consuming to run full experiments multiple times on ImageNet-1k dataset.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    %\answerTODO{}
    \answerYes{See the supplementary material.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    %\answerTODO{}
    \answerYes{}
  \item Did you mention the license of the assets?
    %\answerTODO{}
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    %\answerTODO{}
    \answerYes{See the supplementary material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    %\answerTODO{}
    \answerYes{All the experimental datasets are open source.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    %\answerTODO{}
    \answerNo{Since we only used existing open source datasets we did not add a separate discussion about this.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    %\answerTODO{}
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    %\answerTODO{}
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    %\answerTODO{}
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sota_comparison.tex <==

\begin{table}[t]
\caption{
Comparison to state-of-the-art quantized and binary CNNs on ImageNet \cite{imagenet_cvpr09}.
The bitwidths given represent the precision of: weights (W), activations (A), and the feature map (F).
% All models were trained with cross-entropy loss.
% All models except CI-Net \cite{Wang_2019_CVPR} were trained with a simple cross-entropy loss.
% Methods include low-bit quantization (first section) and approaches with multiple binary bases (second section).
% The comparison is in parallel for two size categories (with differing number of layers).
% The best result in each section is bold.
}
\begin{small}
\begin{center}
\begin{tabular}{|c|c|@{\hskip 0.1cm}|c|c|c|}
\hline
% table head
\thead{Method} & \thead{Bitwidth\\(W/A/F)} & \thead{Top-1\\Acc.} & \thead{Model\\Size} & \thead{OPs\\$(\cdot10^8)$} \\ \hline
32-bit ResNet baseline                          & 32/32/32          & 69.3 &         46.8MB       & 18.1       \\ \hline
BWN\cite{Rastegari2016}                         & 1/32/32           & 60.8 &          4MB         & 18.1       \\
TTQ\cite{zhu2016trained}                        & 2/32/32           & 66.6 &         5.3MB        & 18.1       \\
HWGQ\cite{cai2017deep}                          & 1/2/32            & 59.6 &          4MB         & $\sim$2.4  \\
LQ-Net\cite{zhang2018lq}                        & 1/2/32            & 62.6 &          4MB         & $\sim$2.4  \\
SYQ\cite{faraone2018syq}                        & 1/2/32            & 55.4 &          4MB         & $\sim$2.4  \\
DoReFa\cite{Zhou2016}                           & 2/2/32            & 62.6 &         5.3MB        & $\sim$2.4  \\ \hline
Ensemble\cite{Zhu_2019_CVPR}                    & (1/1/32)$\times$6 & 61.0 &           -          &  -         \\
Circulant-CNN\cite{Cvpr2019}                    & (1/1/32)$\times$4 & 61.4 &           -          &  -         \\
ABC-Net\cite{Lin2017}                           & (1/1/32)$\times$5 & 65.0 &        8.7MB         & 7.8        \\
GroupNet\cite{Lin2017}                          & (1/1/32)$\times$5 & 67.0 &        9.2MB         & 2.68       \\ \hline
BNN\cite{Courbariaux2016}                       & 1/1/32            & 42.2 & \mrc{09}{4MB}        & 1.57       \\
XNOR-Net\cite{Rastegari2016}                    & 1/1/32            & 51.2 &                      & 1.59       \\
Bi-RealNet\cite{Liu_2018_ECCV}                  & 1/1/32            & 56.4 &                      & 1.63       \\
XNOR-Net++\cite{bulat2019xnor}                  & 1/1/32            & 57.1 &                      & 1.59       \\
BinaryDenseNet\cite{Bethge_2019_ICCV_Workshops} & 1/1/32            & 60.7 &                      & 2.58       \\
Strong Baseline\cite{Martinez2020Training}      & 1/1/32            & 60.9 &                      & 1.82       \\
MeliusNetA\cite{}                               & 1/1/32            & 63.4 &                      & 1.62       \\
Real-to-Binary\cite{Martinez2020Training}       & 1/1/32            & 65.4 &                      & 1.83       \\
ReActNet (ResNet)\cite{}                        & 1/1/32            & 65.9 &                      & 1.83       \\ \hline
Ours (ResNet)                                   & 1/1/1             & 48.9 &                      & x       \\
Ours (ResNet)                                   & 1/1/4             & 55.1 &                      & x       \\
Ours (BoolNet)                                  & 1/1/4             & 5x.x &                      & x       \\
Ours (BoolNet)$^*$                              & 1/1/4$^*$         & 6x.x &                      & x       \\ \hline
\end{tabular}\\
{\small $^*$ In this model we use dilation in the last stage of the network.}
% \vspace{-0.6cm}
\end{center}
\end{small}
\label{tab:imagenet-sota}
\end{table}


% \begin{tabular}{|c|c|@{\hskip 0.1cm}|c|c|c|@{\hskip 0.1cm}|c|c|c|}
% \hline
% % table head
% \mrc{3}{Method} & \mrc{3}{Bitwidth\\(W/A)} & \multicolumn{3}{c|@{\hskip 0.1cm}|}{ImageNet ($\approx$18 layers)} & \multicolumn{3}{c|}{ImageNet ($\approx$34 layers)} \\ \cline{3-8}
% & & \thead{Top-1\\Acc.} & \thead{Model\\Size} & \thead{OPs\\$(\cdot10^8)$} & \thead{Top-1\\Acc.} & \thead{Model\\Size} & \thead{OPs\\$(\cdot10^8)$} \\ \hline
% BWN\cite{Rastegari2016}                         & 1/32           & 60.8          &          4MB         & 18.1        & -             &           -           &  -         \\
% TTQ\cite{zhu2016trained}                        & 2/32           & \textbf{66.6} &         5.3MB        & 18.1        & -             &           -           &  -         \\
% HWGQ\cite{cai2017deep}                          & 1/2            & 59.6          &          4MB         & $\sim$2.4   & 64.3          &          5.1MB        & $\sim$3.4  \\
% LQ-Net\cite{zhang2018lq}                        & 1/2            & 62.6          &          4MB         & $\sim$2.4   & \textbf{66.6} &          5.1MB        & $\sim$3.4  \\
% SYQ\cite{faraone2018syq}                        & 1/2            & 55.4          &          4MB         & $\sim$2.4   & -             &           -           &  -         \\
% DoReFa\cite{Zhou2016}                           & 2/2            & 62.6          &         5.3MB        & $\sim$2.4   & -             &           -           &  -         \\ \hline\hline
% Ensemble\cite{Zhu_2019_CVPR}                    & (1/1)$\times$6 & 61.0          &           -          &  -          & -             &           -           &  -         \\
% Circulant-CNN\cite{Cvpr2019}                    & (1/1)$\times$4 & 61.4          &           -          &  -          & -             &           -           &  -         \\
% ABC-Net\cite{Lin2017}                           & (1/1)$\times$5 & 65.0          &        8.7MB         & 7.8         & -             &           -           &  -         \\
% GroupNet\cite{Lin2017}                          & (1/1)$\times$5 & \textbf{67.0} &        9.2MB         & 2.68        & \textbf{70.5} &         15.3MB        & 4.13       \\ \hline\hline
% BNN\cite{Courbariaux2016}                       & 1/1            & 42.2          & \mrc{09}{$\sim$4MB}  & 1.57        & -             & \mrc{09}{$\sim$5.1MB} &  -         \\
% XNOR-Net\cite{Rastegari2016}                    & 1/1            & 51.2          &                      & 1.59        & -             &                       &  -         \\
% Bi-RealNet\cite{Liu_2018_ECCV}                  & 1/1            & 56.4          &                      & 1.63        & 62.2          &                       & 1.93       \\
% XNOR-Net++\cite{bulat2019xnor}                  & 1/1            & 57.1          &                      & 1.59        & -             &                       &  -         \\
% Bi-RealNet\,(our baseline)                      & 1/1            & 60.6          &                      & 1.14        & 63.7          &                       & 1.43       \\
% BinaryDenseNet\cite{Bethge_2019_ICCV_Workshops} & 1/1            & 60.7          &                      & 2.58        & 62.5          &                       & 2.71       \\
% Strong Baseline\cite{Martinez2020Training}      & 1/1            & 60.9          &                      & 1.82        & -             &                       &  -         \\
% BinaryDenseNet\,(our baseline)                  & 1/1            & 62.6          &                      & 2.09        & 64.2          &                       & 2.20       \\
% MeliusNetA,B\,(ours)                            & 1/1            & \textbf{63.4} &                      & 1.62        & \textbf{65.7} &                       & 1.96       \\ \hline\hline
% 32-bit baseline (ResNet)                        & 32/32          & 69.3          &            46.8MB    & 18.1        & 73.3          &            87.2MB     & 36.6       \\ \hline
% \end{tabular}\\

==> sota_curves.tex <==
\begin{figure}[]
\captionsetup[subfigure]{justification=centering}
\begin{center}
\includegraphics[width=\textwidth]{sota_wide.pdf}
\end{center}
\caption{The training and validation accuracy curves of our trainings for the comparison to the state-of-the-art BNNs.}
\label{fig:sota_curves}
\end{figure}

